Circular Belief Propagation for Approximate Probabilistic Inference

Belief Propagation (BP) is a simple probabilistic inference algorithm, consisting of passing messages between nodes of a graph representing a probability distribution. Its analogy with a neural network suggests that it could have far-ranging applications for neuroscience and artificial intelligence. Unfortunately, it is only exact when applied to cycle-free graphs, which restricts the potential of the algorithm. In this paper, we propose Circular Belief Propagation (CBP), an extension of BP which limits the detrimental effects of message reverberation caused by cycles by learning to detect and cancel spurious correlations and belief amplifications. We show in numerical experiments involving binary probabilistic graphs that CBP far outperforms BP and reaches good performance compared to that of previously proposed algorithms.

==> Gaussian_CBP.tex <==
\section{Gaussian Circular BP}\label{sec:gaussian-CBP}

In this section, we present Gaussian CBP and results from supervised learning in Gaussian graphical models.

% ICML\footnote{Remove the simulations of Gaussian CBP (showing the effects of circularity on the means and precisions) and keep only the learning}
Along the way, we also describe the effects of circularity by comparing Gaussian Circular BP to Gaussian BP. Similarly to the binary case where circularity lead to overconfidence, estimates of probabilities are overconfident (as measured by the inverse variance or precision). However, and contrary to the binary case, the MAP estimation (as measured by the mean of the distribution) also gets strongly modified by circularity (it is also the case in the binary case, but only rarely). Simulations show that the means are in general overestimated. % with respect to zero.



% In the main text, we hypothesize that the distribution $p(x)$ only has pairwise factors and that variables are binary (we also impose the pairwise factors to have a particular form corresponding to an Ising model, for the parallel with the classical tanh model). Here, we consider instead the case where the distribution $p(x)$ only has pairwise factors and that variables are Gaussian.


In all this work with the exception of the present section, variables $x_i$ of the probability distribution $p(x_1, \dots, x_n)$ are assumed to be binary variables: $x_i \in \{-1;+1\}$. Equations \eqref{eq:eCBP-message-log} and \eqref{eq:eCBP-belief-log} relate (the log-transforms of) the means of the belief distribution to the ones of the message distribution.

However, many problems involve continuous variables.
In this section, we consider instead the Gaussian case, which is an example of continuous distribution commonly considered. 
We show that the Circular BP algorithm translates into relations between the parameters (mean and variance) of the beliefs and the parameters (mean and variance) of the messages, very similarly to the binary case.

% Work related (to read and cite):
% \begin{itemize}
    % \item \href{https://dspace.mit.edu/bitstream/handle/1721.1/60177/681902681-MIT.pdf?sequence=2}{this master thesis from MIT} (I did not get the Equation (2.13) to (2.17))
    % \item Most importantly, \href{http://ssg.mit.edu/ssg_theses/ssg_theses_2000_2009/Malioutov_PhD_6_08.pdf}{Malioutov's PhD thesis} \citep{Malioutov2008}
    % \item Inference algorithm (I suppose BP) for HMM: see the following article \href{http://mlg.eng.cam.ac.uk/zoubin/papers/lds.pdf}{"A unifying review of linear gaussian models"} from Roweis and Ghahramani
    % \item Work from Weiss (e.g. \citet{Weiss1999}
    % \item \href{https://sci-hub.tw/https://doi.org/10.1162/0899766041941943}{intro of this article from Heskes}: "In gaussian graphical models, the means are guaranteed to coincide with the exact means (Weiss \& Freeman, 2001)")
    % \item Work from Plarre \citep{Plarre2004}
    % \item \citet{Raju2016}
    % \item Work from Pitkow \href{https://www2.securecms.com/CCNeuro/docs-0/5928b63368ed3f69508a255b.pdf}{"Inferring inference"}
    % \item Gaussian EP [The EP Energy Function and Minimization Schemes, Minka 2001], [Expectation Propagation for Approximate Bayesian Inference, Minka 2001]
    % \item $\alpha-BP$ [$\alpha$-Belief propagation as fully factorized approximation, Liu et al, 2019] + 2020 article
% \end{itemize}


\subsection{Circular BP in Gaussian Markov Random Fields}

\subsubsection{Gaussian Markov Random Fields}\label{subsubsec:gaussian-MRF}

We consider in this section a Gaussian Markov Random Field, which is by definition a Markov Random Field (MRF) in which the joint distribution is Gaussian:
\begin{equation}
    p(x) = \sqrt{\frac{|P|}{(2\pi)^n}} \exp\Big(-\frac{1}{2} (x-\mu)^T P (x-\mu)\Big)
\end{equation}
and is commonly used in the fields of computer vision and sensor networks, for instance. The distribution is parametrized by its mean $\mu = \mathbb{E}[x]$ and its \emph{precision matrix} $P$. $P$ is the inverse covariance matrix: $P = \Sigma^{-1}$ where the covariance matrix is $\Sigma = \mathbb{E}[(x-\mu) (x-\mu)^T]$. Matrix $P$ is also known as the \emph{information matrix}, as its sparsity exactly matches the corresponding graphical model: $P_{ij} = 0$ indicates an absence of edge between nodes $i$ and $j$ in the graph.

We use a slightly different parametrization of the Gaussian distribution with its natural parameters $(P, v)$ where $v \equiv P \mu$ is often called the \emph{potential vector} \citep{Raju2016}, instead of using parameters $P$ and $\mu$:
\begin{equation}
    p(x) \propto \exp\Big(-\frac{1}{2} x^T P x + v^T x\Big)
\end{equation}
%The couple $(P, h)$ constitutes in fact the natural parameters of the Gaussian distribution . %notation used for the potential vector: h (?) ; b (Raju)

We assume, as for the binary case, that the probability distribution can be written as a factor of pairwise interactions and unitary interactions:
\begin{equation}
    p(x) = \frac{1}{Z} \prod\limits_{(i,j)} \psi_{ij}(x_i,x_j) \prod\limits_i \psi_i(x_i)
\end{equation}
where potentials have the following Gaussian expression (see section \ref{subsubsec:dem-gaussian-CBP}):
\begin{empheq}[left=\empheqlbrace]{align}
  &\psi_{ij}(x_i, x_j) = \exp\Big(-\frac{1}{2} \begin{pmatrix} x_i\\ x_j\\ \end{pmatrix}^T P_{x_i,x_j} \begin{pmatrix} x_i\\ x_j\\ \end{pmatrix}\Big)\label{eq:phi_ij-gaussian} %(x_i x_j)^T
  \\
  &\psi_i(x_i) = \exp\Big(-\frac{1}{2} P_{\text{ext} \to i} x_i + v_i x_i\Big) %\exp\Big(-\frac{1}{2} P_{\text{ext} \to i} (x_i-\mu_{\text{ext} \to i})^2\Big)
\end{empheq}
where $P_{x_i,x_j} \equiv \begin{pmatrix}
P_{x_i,x_j}^{x_i,x_i} & P_{x_i,x_j}^{x_i,x_j}\\
P_{x_i,x_j}^{x_j,x_i} & P_{x_i,x_j}^{x_j,x_j}
\end{pmatrix}$ is a $2\times2$ matrix.

Note that Equation \ref{eq:phi_ij-gaussian} is equivalent to writing $x_i = C x_j + N$ where $N$ is Gaussian noise with zero mean (with $C = - P_{x_i,x_j}^{x_i,x_j}/P_{x_i,x_j}^{x_i,x_i}$ and precision $P_{x_i,x_j}^{x_i,x_i}$ for $N$).


\subsubsection{BP in Gaussian graphical models}

The Belief Propagation algorithm has been studied empirically and theoretically in the Gaussian case specifically; see for instance \citet{Malioutov2008}. It is also the case for extensions of BP like Expectation Propagation \citep{Minka2001a, Minka2001b}, Fractional Belief Propagation \citep{Cseke2011} and $\alpha$-BP \citep{Liu2020}. When applied on probabilistic graphs with cycles, Belief Propagation often performs reasonably well. As shown in \citet{Weiss1999}, when the algorithm converges it produces the correct means, but generally not the correct variances. A nice example of application of Belief Propagation in Gaussian Markov Random Fields is provided in \citet{Weiss1997}, where BP is used to estimate the direction of motion automatically given a video of a hand moving.
% \afterPhD{Gaussian BP minimizes the MSE = "Minimum mean-squared error" (see "Learning Motion Analysis" (Freeman et al, 2000) and its references 31,40,22)}

\subsubsection{Formulation of Circular BP in Gaussian MRF}

In the case described in the above section \ref{subsubsec:gaussian-MRF}, marginals $\{p_i(x_i)\}$ of the distribution can be approximated using BP and its extension, the Circular BP algorithm. Circular BP consists of very simple update equations on the parameters of the distribution, by sending (as in the binary case) messages between nodes of the graph to spread information to all nodes.
The relations between the mean $\mu_i$ (or rather the potential vector $v_i \equiv P_i \mu_i$) and precision $P_i$ of the beliefs and the mean $\mu_{i \to j}$ and precision $P_{i \to j}$ of the messages are the following (see the following section for a demonstration):\footnote{Note that all the parameters in Equations \eqref{eq:eCBP-message-precision-gaussian}-\eqref{eq:function-h_ij} are scalars.}%\footnote{Choose which version to show ($f$ or $f_1$).}
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_{i \to j}^{\text{new}} = g_{ij}(P_i - \alpha_{ij} P_{j \to i}) \label{eq:eCBP-message-precision-gaussian}
  \\
  &v_{i \to j}^{\text{new}} =  h_{ij}\Big(v_i - \alpha_{ij} v_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}  \Big) \label{eq:eCBP-message-mean-gaussian} %P_{i \to j}^{\text{new}} \mu_{i \to j}^{\text{new}} =  h_{ij}\Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}  \Big)
\end{empheq}
% \end{subequations}
% \begin{subequations}
where
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_i = \kappa_i \Big(\sum\limits_{j \in N(i)} P_{j \to i} + \gamma_i P_{\text{ext} \to i}  \Big)
  \label{eq:eCBP-belief-precision-gaussian} %P_{x_i | y_i}
  \\
  &v_i = \kappa_i \Big( \sum\limits_{j \in N(i)} v_{j \to i} + \gamma_i v_{\text{ext} \to i}\Big) \label{eq:eCBP-belief-mean-gaussian} % - P_{x_i,y_i}^{x_i,y_i} y_i   %P_{x_i | y_i} %\mu_{x_i | y_i}  %P_i \mu_i = \kappa_i \Big( \sum\limits_{j \in N(i)} P_{j \to i} \mu_{j \to i} + \gamma_i P_{\text{ext} \to i}  \mu_{\text{ext} \to i}\Big)
\end{empheq}
% \end{subequations}
and where functions $g_{ij}$ and $h_{ij}$ are given by
\begin{equation}
    g_{ij}(y) = \beta_{ij} P_{x_i,x_j}^{x_j,x_j} - \frac{(\beta_{ij} P_{x_i,x_j}^{x_i,x_j})^2}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + y}
\end{equation}
and 
\begin{equation}\label{eq:function-h_ij}
    h_{ij}(x,y) = - \frac{\beta_{ij} P_{x_i,x_j}^{x_i,x_j} x}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + y}
\end{equation}
% or equivalently,
% \begin{equation}
%     P_{i \to j} \mu_{i \to j} = \tilde{h}_{ij} \Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i}, P_{i \to j})
% \end{equation}
% where
% \begin{equation}
%     \tilde{h}_{ij}(x, y) = \frac{x}{\beta_{ij} P_{x_i, x_j}^{x_i, x_j}} (\beta_{ij} P_{x_i,x_j}^{x_j, x_j} - y)
% \end{equation}
%In what follows, we consider that all variables have dimension $n = 1$ for simplicity (thus all variables and parameters in the equations below are scalars).

These equations logically extend the ones obtained for BP (see for instance \citet{Weiss1999, Plarre2004}) for which parameters ($\bm{\alpha}, \bm{\kappa}, \bm{\beta}, \bm{\gamma}$) take value $\bm{1}$. %\footnote{See for Plarre2004 in my Latex document about Circular BP in Gaussian GM --> check} --> ok

\paragraph{Similarity with the binary case}
Equations \eqref{eq:eCBP-message-precision-gaussian} and \eqref{eq:eCBP-message-mean-gaussian}, which relate the parameters $(P_{i \to j},\, v_{i \to j})$ of the message distribution to the parameters $(P_{i},\, v_{i})$ of the marginal distribution and the parameters $(P_{j \to i},\, v_{j \to i})$ of the opposite message distribution, have exactly the same form as in the binary case, with the subtraction of the ``belief variable" by the ``opposite message variable" with weight $\alpha_{ij}$ ($M_{i \to j} = f_{ij}(B_i - \alpha_{ij} M_{j \to i}) \equiv f(B_i - \alpha_{ij} M_{j \to i}, \beta_{ij} J_{ij})$). Indeed, in the binary case, the evolution of the only parameter of the message distribution (its expected value $m_{i \to j}(x_j=+1)$, or rather, the transform $M_{i \to j} \equiv \frac{1}{2} \log\big(\frac{m_{i \to j}(x_j=+1)}{m_{i \to j}(x_j=-1)}\big)$) is expressed as a function of a quantity associated to the marginal distribution $B_i \equiv \frac{1}{2} \log\big(\frac{b_i(x_i=+1)}{b_i(x_i=-1)}\big)$ and the parameter of the opposite message distribution $M_{j \to i}$ weighted by $\alpha_{ij}$ as $M_{i \to j} = f_{ij}(B_i - \alpha_{ij} M_{j \to i})$. In both the Gaussian and the binary case, the quantity associated to the marginal distribution gets subtracted by $\alpha_{ij}$ times the quantity associated to the message distribution (for the message going in the opposite direction).
As a reminder, the sign of function $f$ used in the binary case is determined by the interaction between $x_i$ and $x_j$ ($J_{ij}>0$ indicates a positive interaction) and the sign of its argument. Similarly, the sign of $h_{ij}$ depends on the sign of its first argument, as well as the sign of the interaction between variables $x_i$ and $x_j$ (a positive interaction means that $P_{x_i,x_j}^{x_i,x_j} <0$ as the precision is the inverse covariance). Function $g_{ij}$ is positive as precision matrices are positive definite and symmetrical matrices by definition. $g_{ij}$ is an increasing function of its argument $P_i - \alpha_{ij} P_{j \to i}$. The absolute value of function $h_{ij}$, $\abs{h_{ij}}$, increases as function of its first argument $v_i - \alpha_{ij} v_{j \to i}$ and decreases as function its second argument $P_i - \alpha_{ij} P_{j \to i}$.

Likewise, Equations \eqref{eq:eCBP-belief-precision-gaussian} and \eqref{eq:eCBP-belief-mean-gaussian} giving the expression of the (transform of the) marginal distribution parameter are similar to the expression in the binary case $B_i = \kappa_i \Big(\sum_{j \in \mathcal{N}(i)} M_{j \to i} + \gamma_i M_{\text{ext} \to i}\Big)$. The variable of interest associated to node $i$ (function of the parameter(s) of the $b_i(x_i)$) is the sum of all the contributions from its neighbors and from the external world.

Running these equations iteratively (see Algorithm \ref{alg:gaussian-ecbp-pairwise}) allows one, as in the binary case, to marginalize the distribution. In the Gaussian case, this means obtaining estimates of the mean and variance of the variables $\{x_i\}$, given the external information $\{\psi_i(x_i)\}$ (through $\{P_{\text{ext} \to i}\}$ and $\{\mu_{\text{ext} \to i}\}$) %(through $\{P_{x_i | y_i}\}$ and $\{\mu_{x_i | y_i}\}$)
and the conditional dependencies between variables $\{\psi_{ij}(x_i,x_j)\}$ (through $\{P_{x_i,x_j}\}$).

\paragraph{Equivalent formulation of Gaussian Circular BP}
We also write an equivalent formulation of the algorithm, which first consists of running the updates on precisions and only then on potential vectors (or equivalently, on means). Indeed, in the equations above, precisions $\{P_i\}$ and $\{P_{i \to j}\}$ do not depend on the potentials $\{v_i\}$ and $\{v_{i \to j}\}$. %Indeed, in the equations above, precisions $\{P_i\}$ and $\{P_{i \to j}\}$ do not depend on the strength of the external inputs $\{\mu_{\text{ext} \to i}\}$ (or equivalently, $\{\mu_{\text{ext} \to i}\}$). %Instead, they only depend on the graph structure, the $\bm{\alpha}$, $\bm{\kappa}$, $\bm{\beta}$ and $\bm{\gamma}$ parameters and the precisions associated to the external inputs $\{P_{\text{ext} \to i}\}$ %$\{P_{x_i | y_i}\}$
%and to the edges $\{P_{x_i,x_j}\}$, all of which being fixed parameters. % even in a context where external inputs are variable (in this case, what varies is the means $\{\mu_{\text{ext} \to i}\}$ %$\{\mu_{x_i | y_i}\}$
%but not the precisions $\{P_{\text{ext} \to i}\}$). %$\{P_{x_i | y_i}\}$
Thefore, precisions can be computed at first and fixed once for all, and the ``real" algorithm would consist in running the updates on the means with potentially time-varying inputs $\{\mu_{\text{ext} \to i}\}$. %$\{\mu_{x_i | y_i}\}$
By writing $\mu = (P \mu) / P = v / P$, we obtain after some mathematical manipulations the following update equations on the means:
% \begin{equation}
%     \mu_i = \frac{\sum\limits_{j \in N(i)} P_{j \to i} \mu_{j \to i} + \gamma_i P_{x_i | y_i}  \mu_{x_i | y_i}}{\sum\limits_{j \in N(i)} P_{j \to i} + \gamma_i P_{x_i | y_i}}
% \end{equation}
% \begin{equation}
%     \mu_{i \to j} =  \frac{f \Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}  \Big)}{g(P_i - \alpha_{ij} P_{j \to i})}
% \end{equation}
% \begin{equation}
%     = \frac{- P_{x_i,x_j}^{x_i,x_j} (P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i})}{\beta_{ij} [P_{x_i,x_j}^{x_j,x_j}  P_{x_i,x_j}^{x_i,x_i}  -  (P_{x_i,x_j}^{x_i,x_j}]^2) +  P_{x_i,x_j}^{x_j,x_j} (P_i - \alpha_{ij} P_{j \to i})}
% \end{equation}
% which leads to
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &\mu_i = \sum\limits_{j \in N(i)} k_{j \to i} \mu_{j \to i} + k_{\text{ext} \to i} \mu_{\text{ext} \to i} \label{eq:mean-marginal-gaussian}\\ %k_{x_i | y_i} \mu_{x_i | y_i}
  &\mu_{i \to j}^{\text{new}} = h_i \mu_i - h_{j \to i} \mu_{j \to i} \label{eq:mean-message-gaussian}
\end{empheq}%\afterPhD{To be compared with the Kalman filter equations?}%\afterPhD{Form of divisive inhibition? See refs 14,13 of Wilson2009}
% \end{subequations}
with coefficients $k_{j \to i} \equiv \cfrac{P_{j \to i}}{\sum\limits_{j \in N(i)} P_{j \to i} + \gamma_i P_{\text{ext} \to i}}$\,,\, %P_{x_i | y_i}}
$k_{\text{ext} \to i} \equiv \cfrac{\gamma_i P_{\text{ext} \to i}}{\sum\limits_{j \in N(i)} P_{j \to i} + \gamma_i P_{\text{ext} \to i}}$%k_{x_i | y_i} %P_{x_i | y_i}
\,,\\ $h_i \equiv \cfrac{-P_{x_i,x_j}^{x_i,x_j} P_i}
{\beta_{ij} |P_{x_i,x_j}| +  P_{x_i,x_j}^{x_j,x_j} (P_i - \alpha_{ij} P_{j \to i})}$\,, and 
$h_{j \to i} \equiv \cfrac{- P_{x_i,x_j}^{x_i,x_j} \alpha_{ij} P_{j \to i} }{\beta_{ij} |P_{x_i,x_j}| +  P_{x_i,x_j}^{x_j,x_j} (P_i - \alpha_{ij} P_{j \to i})}$. %"|P_{x_i,x_j}|" instead of"P_{x_i,x_j}^{x_j,x_j}  P_{x_i,x_j}^{x_i,x_i}  -  (P_{x_i,x_j}^{x_i,x_j})^2" because P_{x_i,x_j} is a symmetric matrix as it is a precision matrix (inverse of a covariance matrix, which is by definition symmetric: see wikipedia for instance)
Coefficients $\{k_{j \to i}\}$ and $k_{\text{ext} \to i}$ are positive and sum to 1. Coefficients $h_i$ and $h_{j \to i}$ can be positive or negative, and their difference or sum is not equal to 1 in general (however, they have identical signs for $\alpha_{ij} > 0$ which is a reasonable hypothesis, and they are positive if $x_i$ and $x_j$ positively interact, that is, $P_{x_i,x_j}^{x_i,x_j} < 0$, and for a ``reasonable" choice of parameters). %are both positive if $0<\alpha_{ij}<1$ and $\kappa<1$).


\begin{algorithm}
\caption{Gaussian Circular BP algorithm in a pairwise factor graph} \label{alg:gaussian-ecbp-pairwise}
\begin{algorithmic}[1]
% \Input
% \Output
%\STATE \SET \{\psi_{ij}(x_i,x_j)\}, \{\psi_{i}(x_j)\}
\FORALL{directed edges $i \to j$}
    \STATE $P_{i \to j} \gets$ random positive value \hfill\COMMENT{Initialize the messages' precisions}
    \STATE $v_{i \to j} \gets$ random value \hfill\COMMENT{Initialize the messages' potentials} %means $\times$ precisions} %$\mu_{i \to j}
\ENDFOR
\REPEAT
    \FORALL{nodes $x_i$}
        \STATE $P_i = \kappa_i \Big(\sum\limits_{j \in N(i)} P_{j \to i} + \gamma_i P_{\text{ext} \to i}  \Big)$ \hfill\COMMENT{Compute the beliefs' precisions} %P_{x_i | y_i} 
        \STATE $v_i = \kappa_i \Big( \sum\limits_{j \in N(i)} v_{j \to i} + \gamma_i v_{\text{ext} \to i}\Big)$ \hfill\COMMENT{Compute the beliefs' potentials} %means\\\hfill $\times$ precisions} %P_{x_i | y_i}  \mu_{x_i | y_i}  %$P_i \mu_i = \kappa_i \Big( \sum\limits_{j \in N(i)} P_{j \to i} \mu_{j \to i} + \gamma_i P_{\text{ext} \to i}  \mu_{\text{ext} \to i}\Big)$
    \ENDFOR
    \FORALL{directed edges $x_i \to x_j$}
        \STATE $P_{i \to j}^{\text{new}} = g_{ij}(P_i - \alpha_{ij} P_{j \to i})$ \hfill\COMMENT{Update the messages' precisions} 
        \STATE $v_{i \to j}^{\text{new}} =  h_{ij}\Big(v_i - \alpha_{ij} v_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}  \Big)$ \hfill\COMMENT{Update the messages' potentials} %means\\\hfill $\times$ precisions}  %$P_{i \to j}^{\text{new}} \mu_{i \to j}^{\text{new}} =  h_{ij}\Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}  \Big)$
    \ENDFOR
    \STATE $P \gets  P^{\text{new}}$
    \STATE $\mu \gets  \mu^{\text{new}}$
\UNTIL convergence %or maximum iteration
\FORALL{nodes $x_i$}
    \STATE $b_i(x_i) \gets \sqrt{\cfrac{P_i}{2 \pi}} \exp\Big(-\cfrac{1}{2} P_i x_i^2 + v_i x_i\Big)$ \hfill\COMMENT{Compute the beliefs} %$b_i(x_i) \gets \sqrt{\cfrac{P_i}{2 \pi}} \exp\Big(-\frac{1}{2} (x_i-\mu_{i})^T P_{i} (x_i- \mu_{i})\Big)$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsubsection{Demonstration}\label{subsubsec:dem-gaussian-CBP}
Here we demonstrate the equations \eqref{eq:eCBP-message-precision-gaussian}-\eqref{eq:function-h_ij} which describe Circular BP in the Gaussian case.

\paragraph{Mean and precision of messages}
We start by writing the message update equation for Circular Belief Propagation (the integral replaces the sum as $x$ takes continuous values):
\begin{equation}
  m_{i \to j}(x_j)
   \propto \int\limits_{x_i} \psi_{i,j}(x_i,x_j)^{\beta_{ij}} \Bigg[\prod\limits_{k \in N(i) \setminus j} m_{k \to i}(x_i) \: m_{y_i \to x_i}(x_i)^{\gamma_i} \Big( m_{j \to i}(x_i) \Big)^{1-\alpha_{ij}/\kappa_i}\Bigg]^{\kappa_i} dx_i
\end{equation}
Here we hypothesize that messages have a normal distribution. We use, by slight abuse of notation, $\mathcal{N}$ to denote the density of the normal distribution (and not the law): $ \mathcal{N}_{x}(\mu,\, P) \equiv \sqrt{\abs{P}/(2 \pi)} \times \exp\Big(-\frac{1}{2} (x-\mu)^T P (x- \mu)\Big)$ where $\mu$ is the mean of the distribution and $P = \Sigma^{-1}$ is the precision matrix or inverse covariance matrix (note that here we consider for simplicity that all variables $x_i$ have dimension 1, thus $\mu_{i \to j}, \mu_i$, $P_{i \to j}$ and $P_i$ are scalars). The message distribution is thus written:
\begin{equation}
    m_{i \to j}(x_j) = \mathcal{N}_{x_j}(\mu_{i \to j},\, P_{i \to j})
\end{equation}
We also hypothesize that the potentials have a normal distribution. %\footnote{If I want to add something about the decomposition of factors, see my latex document about Circular BP in Gaussian graphical models} 
As in \citet{Weiss1999}, we assume, without loss of generality, that the joint means are zero:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &\psi_{ij}(x_i, x_j) = \mathcal{N}_{(x_i, x_j)}(0,\, P_{x_i, x_j})%\label{} %\quad \text{where } X_{ij} = (x_i, x_j)  %\exp \Bigg(-\frac{1}{2} \begin{pmatrix} x_i\\ x_j \end{pmatrix}^T P_{x_i,x_j}\begin{pmatrix} x_i\\ x_j \end{pmatrix} \Bigg)
  \\
  &\psi_i(x_i) = m_{y_i \to x_i}(x_i) = \mathcal{N}_{(x_i, y_i)}(0, P_{x_i, y_i}) \propto \mathcal{N}_{x_i}(\mu_{x_i | y_i},\, P_{x_i | y_i}) \label{eq:univ-potential-gaussian} %\sim \mathcal{N}_{X_i}(0, P_{X_i}) \quad \text{where } X_{i} = (x_i, y_i)
\end{empheq}
% \end{subequations}
where $y_i$ is a noisy observation related to $x_i$ only, $P_{x_i,x_j}$ and $P_{x_i,y_i}$ are 2x2 matrices, and the parameters of the Gaussian distribution in Equation \eqref{eq:univ-potential-gaussian} are given by $P_{x_i,y_i}^{x_i,x_i} \times \mu_{x_i | y_i} = -P_{x_i,y_i}^{x_i,y_i}\times y_i$ and $P_{x_i | y_i} = P_{x_i,y_i}^{x_i,x_i}$ (conditional distribution). In the following, $P_{x_i | y_i}$ is written $P_{\text{ext} \to i}$ and $\mu_{x_i | y_i}$ is written $\mu_{\text{ext} \to i}$.  %The proportionality constant does not depend on $x_i$ (but depends on variable $y_i$, which takes its observed value).
\begin{align} 
  \implies m_{i \to j}(x_j)  \propto & \int\limits_{x_i} \mathcal{N}_{(x_i, x_j)}(0, P_{x_i, x_j})^{\beta_{ij}}
\Bigg[\prod\limits_{k \in N(i) \setminus j} \mathcal{N}_{x_i}(\mu_{k \to i},P_{k \to i}) \: 
\mathcal{N}_{x_i}(\mu_{\text{ext} \to i}, P_{\text{ext} \to i})^{\gamma_i}\notag \\
&\times \mathcal{N}_{x_i}(\mu_{j \to i},P_{j \to i})^{1-\alpha_{ij}/\kappa_i}\Bigg]^{\kappa_i} dx_i
\end{align}
Using the fact that $\big( \mathcal{N}_x(\mu,P) \big) ^{k} \propto \mathcal{N}_x(\mu,P \times k)$, it comes:
\begin{align}
  m_{i \to j}(x_j)
 \propto & \int\limits_{x_i} \mathcal{N}_{(x_i, x_j)}(0, \tilde{P}_{x_i, x_j})
\Bigg[\prod\limits_{k \in N(i) \setminus j} \mathcal{N}_{x_i}(\mu_{k \to i},P_{k \to i}) \: 
\mathcal{N}_{x_i}(\mu_{\text{ext} \to i}, \tilde{P}_{\text{ext} \to i}) \notag \\ %\exp \Big(-\frac{1}{2} \begin{pmatrix} x_i\\ x_j \end{pmatrix}^T
\tilde{P}_{x_i,x_j}\begin{pmatrix} x_i\\ x_j \end{pmatrix} \Big)
&\times \mathcal{N}_{x_i}(\mu_{j \to i},(1-\alpha_{ij}/\kappa_i) P_{j \to i})\Bigg]^{\kappa_i} dx_i
\end{align}
where by definition,
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &\tilde{P}_{\text{ext} \to i} = \gamma_i P_{\text{ext} \to i} %\label{}
  \\
  &\tilde{P}_{x_i,x_j} = \beta_{ij} P_{x_i,x_j} %\label{}
\end{empheq}
% \end{subequations}
It comes:
\begin{equation}\label{eq:message-with-integral}
    m_{i \to j}(x_j) \propto \int\limits_{x_i} \exp \Big(-\frac{1}{2} \begin{pmatrix} x_i\\ x_j \end{pmatrix}^T
\tilde{P}_{x_i,x_j}\begin{pmatrix} x_i\\ x_j \end{pmatrix} \Big) \mathcal{N}_{x_i}(\tilde{\mu}_i, \tilde{P}_i) dx_i
\end{equation}
where 
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &\tilde{P}_i \tilde{\mu}_i = \kappa_i \Big(\sum\limits_{k \in N(i) \setminus j} P_{k \to i} \mu_{k \to i} + \tilde{P}_{\text{ext} \to i} \mu_{\text{ext} \to i} + \Big(1-\frac{\alpha_{ij}}{\kappa_i}\Big) P_{j \to i} \mu_{j \to i} \Big) %\label{} %"-\tilde{P}_{x_i,y_i}^{x_i,y_i} y_i" = "\tilde{P}_{x_i | y_i} \mu_{x_i | y_i}"
  \\
  &\tilde{P}_i = \kappa_i \Big(\sum_{k \in N(i) \setminus j} P_{ki} + \tilde{P}_{\text{ext} \to i} + \Big(1-\frac{\alpha_{ij}}{\kappa_i}\Big)P_{j \to i}\Big) %\label{} 
\end{empheq}
% \end{subequations}
(as a product of Gaussian densities: precisions $P$ add up, and precisions multiplied by means $P \mu$ add up as well).\\ %where $\tilde{P}_{x_i,y_i} = \gamma_i P_{x_i,y_i}$.

\noindent We now define
%\footnote{For some reason, in [Weiss and Freeman, 1999], $P_{x_i,y_i}^{x_i,x_i}$ is written $P_{i,i}$ and $-P_{x_i,y_i}^{x_i,y_i} y_i$ is written $P_{i,i}\mu_{i,i}$. --> Can I do that? Why is there a sign difference and one less free variable? Is there a relationship between $\mu_{i,i}$ and $y_i$ (equality / equality with minus sign / proportional with ratio $P_{11}/P_{12}$?} ---> ok: $P_{x_i,y_i}^{x_i,x_i} \mu_{x_i | y_i} = -P_{x_i,y_i}^{x_i,y_i} y_i$ and $P_{x_i | y_i} = P_{x_i,y_i}^{x_i,x_i}$
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_0^{i,j} = \tilde{P}_{x_i,y_i}^{x_i,x_i} + \sum\limits_{k \in N(i) \setminus j} P_{k \to i} %\label{}
  \\
  &P_0^{i,j} \mu_0^{i,j} = \tilde{P}_{\text{ext} \to i} \mu_{\text{ext} \to i} + \sum\limits_{k \in N(i) \setminus j} P_{k \to i} \mu_{k \to i} %\label{}
\end{empheq}
% \end{subequations}
It then comes:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &\tilde{P}_i \tilde{\mu}_i = \kappa_i \Big(P_0^{i,j} \mu_0^{i,j} + \Big(1-\frac{\alpha_{ij}}{\kappa_i}\Big) P_{j \to i} \mu_{j \to i} \Big) %\label{}
  \\
  &\tilde{P}_i = \kappa_i \Big(P_0^{i,j} + \Big(1-\frac{\alpha_{ij}}{\kappa_i}\Big) P_{j \to i} \Big) %\label{}
\end{empheq}
% \end{subequations}
Finally, we write the result of Equation \eqref{eq:message-with-integral}: $m_{i \to j}(x_j)$ is the integral over $x_i$ of the product between a bivariate Gaussian density $\mathcal{N}_{(x_i,x_j)}(0,\tilde{P}_{x_i,x_j})$ and a univariate Gaussian density $\mathcal{N}_{x_i}(\tilde{\mu}_i, \tilde{P}_i)$, thus %(see section \ref{subsec:integral-product-gaussian}) 
the message $m_{i \to j}(x_j)$ has a normal distribution $\mathcal{N}_{x_j}(\mu_{i \to j}, P_{i \to j})$ with the following mean and precision:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_{i \to j} = \cfrac{\tilde{\Sigma}_{x_i,x_j,11} + \frac{1}{\tilde{P}_i}}{|\tilde{\Sigma}_{x_i,x_i}| + \tilde{\Sigma}_{x_i,x_j,22}\frac{1}{\tilde{P}_i}} %\label{}
  \\
  &\mu_{i \to j} = \tilde{\mu}_i \cfrac{\tilde{\Sigma}_{x_i,x_j,12}}{\frac{1}{\tilde{P}_i} + \Sigma_{x_i,x_j,11}} %\label{}
\end{empheq}
% \end{subequations}
It comes:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_{i \to j} = \cfrac{\frac{\tilde{P}_{x_i,x_j,22}}{|\tilde{P}_{x_i,x_j}|} + \frac{1}{\tilde{P}_i}}{\frac{1}{|\tilde{P}_{x_i,x_j}|} + \frac{\tilde{P}_{x_i,x_j,11}}{|\tilde{P}_{x_i,x_j}|}\frac{1}{\tilde{P}_i}} = 
\cfrac{\tilde{P}_{x_i,x_j,22} \tilde{P}_i + |\tilde{P}_{x_i,x_j}|}{\tilde{P}_i + \tilde{P}_{x_i,x_j,11}}
= \tilde{P}_{x_i,x_j,22} - \frac{(\tilde{P}_{x_i,x_j,12})^2}{\tilde{P}_i + \tilde{P}_{x_i,x_j,11}} \notag%\label{}
  \\
  &\mu_{i \to j} = \tilde{P}_i \tilde{\mu}_i \cfrac{-\frac{\tilde{P}_{x_i,x_j,21}}{|\tilde{P}_{x_i,x_j}|}}{1 + \tilde{P}_i \frac{\tilde{P}_{x_i,x_j,22}}{|\tilde{P}_{x_i,x_j}|}}
= - \tilde{P}_i \tilde{\mu}_i \cfrac{\tilde{P}_{x_i,x_j,21}}{|\tilde{P}_{x_i,x_j}| + \tilde{P}_i \tilde{P}_{x_i,x_j,22}}
= - \tilde{P}_i \tilde{\mu}_i \cfrac{\tilde{P}_{x_i,x_j,21}}{P_{i \to j} (\tilde{P}_i + \tilde{P}_{x_i,x_j,11})} \notag%\label{}
\end{empheq}
% \end{subequations}
We thus obtain the following formulas for $P_{i \to j}$ and $\mu_{i \to j}$:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_{i \to j} = \beta_{ij} P_{x_i,x_j}^{x_j,x_j} - \frac{(\beta_{ij} P_{x_i,x_j}^{x_i,x_j})^2}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + \kappa_i \Big(P_0^{i,j} + (1-\alpha_{ij}/\kappa_i)P_{j \to i}\Big)} \label{eq:precision-message-gaussian}
  \\
  &\mu_{i \to j}  = - \frac{\beta_{ij} P_{x_i,x_j}^{x_i,x_j} \kappa_i [P_0^{i,j} \mu_0^{i,j} + (1-\alpha_{ij}/\kappa_i) P_{j \to i} \mu_{j \to i} ]}{P_{i \to j} [\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + P_0^{i,j} + (1-\alpha_{ij}/\kappa_i)P_{j \to i}]} \label{mean-message-gaussian}
\end{empheq}
% \end{subequations}

\paragraph{Mean and precision of the beliefs}
We now write the expression of the beliefs:
\begin{equation}\label{eq:belief-gaussian}
    b_i(x_i) \propto \Bigg(\prod\limits_{j \in N(i)} m_{j \to i}(x_i) \: \psi_i(x_i)^{\gamma_i}\Bigg)^{\kappa_i} %m_{y_i \to x_i}(x_i)
\end{equation}
where 
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &m_{j \to i}(x_i) \propto \mathcal{N}_{x_i}(\mu_{j \to i},\, P_{j \to i}) %\label{}
  \\
  &\psi_i(x_i) \propto \mathcal{N}_{x_i}(\mu_{\text{ext} \to i},\, \Sigma_{\text{ext} \to i}) %\label{} %m_{y_i \to x_i}(x_i)
\end{empheq}
% \end{subequations}
%with $\mu_{x_i | y_i} = -\cfrac{P_{x_i,y_i}^{x_i,y_i} y_i}{P_{x_i,y_i}^{x_i,x_i}}$ and $\Sigma_{x_i | y_i} = \cfrac{1}{P_{x_i,y_i}^{x_i,x_i}}$.
It comes from Equation \eqref{eq:belief-gaussian} that the beliefs follows a Gaussian distribution ($\log(b_i(x_i)) = C -\frac{1}{2} (x-\mu_i)^T P_i (x- \mu_i)$) with precision $P_i$ and mean $\mu_i$ such that:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &P_i = \kappa_i \Big(\sum\limits_{j \in N(i)} P_{j \to i} + \gamma_i P_{\text{ext} \to i} \Big) \label{eq:precision-belief-gaussian} %P_{x_i,y_i}^{x_i,x_i}
  \\
  &P_i \mu_i = \kappa_i \Big( \sum\limits_{j \in N(i)} P_{j \to i} \mu_{j \to i} + \gamma_i P_{\text{ext} \to i} \mu_{\text{ext} \to i}\Big) \label{eq:mean-belief-gaussian} % - P_{x_i,y_i}^{x_i,y_i} y_i   %P_{x_i,y_i}^{x_i,x_i}
\end{empheq}
% \end{subequations}

\paragraph{Relations between means and precisions of the messages and the beliefs}
Here we combine Equations \eqref{eq:precision-message-gaussian} and
\eqref{mean-message-gaussian} giving the expression of the mean and precision of the messages, with Equations \eqref{eq:precision-belief-gaussian} and 
\eqref{eq:mean-belief-gaussian} giving the expression of the mean and precision of the beliefs.
% If we consider the following hypotheses
%\footnote{I think the symmetry of $P_{x_i,y_i}$ and of $P_{x_i, x_j}$ is already needed above...} --> it's actually automatic, because it's covariance matrices --> they are symmetric
% :
% \begin{itemize}
%     \item $P_i, P_{i \to j} > 0$
%     \item $P_{x_i,y_i}^{x_i,x_i}, P_{x_i,y_i}^{y_i,y_i} > 0$
%     \item $P_{x_i,x_j}^{x_i,x_i}, P_{x_i,x_j}^{x_j,x_j} > 0$
%     \item $P_{x_i,y_i}^{x_i,y_i} = P_{x_i,y_i}^{y_i,x_i}  < 0$
%     \item $P_{x_i,x_j}^{x_i,x_j} = P_{x_i,x_j}^{x_j,x_i} < 0$
% \end{itemize}
% then:
% \begin{subequations}
\begin{empheq}[left=\empheqlbrace]{align}%\label{}
  &\kappa_i P_0^{i,j} = P_i - \kappa_i P_{j \to i} %\label{}
  \\
  &\kappa_i P_0^{i,j}\mu_0^{i,j} = \mu_i P_i - \kappa_i \mu_{j \to i} P_{j \to i} %\label{}
\end{empheq}
% \end{subequations}
So $P_0^{i,j} + (1-\frac{\alpha_{ij}}{\kappa_i})P_{j \to i} = \frac{1}{\kappa_i} \Big(P_i - \alpha_{ij} P_{j \to i}\Big)$\\
and $P_0^{i,j}\mu_0^{i,j} + (1-\frac{\alpha_{ij}}{\kappa_i}) P_{j \to i} \mu_{j \to i} = \frac{1}{\kappa_i} \Big( \mu_i P_i - \alpha_{ij} \mu_{j \to i} P_{j \to i}\Big)$

\noindent We thus obtain from Equation \eqref{eq:precision-message-gaussian}:
\begin{align}
    P_{i \to j} &= \beta_{ij} P_{x_i,x_j}^{x_j,x_j} - \frac{(\beta_{ij} P_{x_i,x_j}^{x_i,x_j})^2}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + P_i - \alpha_{ij} P_{j \to i}}\\
    &= g_{ij}(P_i - \alpha_{ij} P_{j \to i} )
\end{align}
where 
% \begin{equation}
    $g_{ij}(y) = \beta_{ij} P_{x_i,x_j}^{x_j,x_j} - \cfrac{(\beta_{ij} P_{x_i,x_j}^{x_i,x_j})^2}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + y}$\,.
% \end{equation}

Similarly, Equation \eqref{mean-message-gaussian} gives:
\begin{align}
    P_{i \to j} \mu_{i \to j}  &= - \frac{\beta_{ij} P_{x_i,x_j}^{x_i,x_j} [P_i \mu_i - \alpha_{ij} \mu_{j \to i} P_{j \to i}]}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + P_i - \alpha_{ij} P_{j \to i}}\\
    &=  h_{ij}\Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}  \Big)
\end{align}
where 
% \begin{equation}
    $h_{ij}(x,y) = - \cfrac{\beta_{ij} P_{x_i,x_j}^{x_i,x_j} x}{\beta_{ij} P_{x_i,x_j}^{x_i,x_i} + y}$\,. \qedwhite
% \end{equation}
% or equivalently,
% % \begin{align}
% %     P_{i \to j} \mu_{i \to j} &= f \Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, g^{-1}(P_{i \to j}) \Big)\\
% %     &\equiv f_1 \Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, P_{i \to j}) 
% % \end{align}
% \begin{equation}
%     P_{i \to j} \mu_{i \to j} = f_1 \Big(P_i \mu_i - \alpha_{ij} P_{j \to i} \mu_{j \to i},\, P_{i \to j}) 
% \end{equation}
% where
% \begin{equation}
%     f_1(x, y) = - \frac{x}{\beta_{ij} P_{x_i, x_j}^{x_i, x_j}} (\beta_{ij} P_{x_i,x_j}^{x_j, x_j} - y)
% \end{equation}
%\footnote{Signs: is $P_{x_i,x_j}^{x_i,x_j}$ necessarily $<0$? In this case, functions $h_{ij}$ and $\tilde{h}_{ij}$ have the same sign as $x$ (otherwise, they have the same sign as $-x / P_{x_i,x_j}^{x_i,x_j}$)} --> actually not even, as the denominator could also be <0 (however, if alpha<=1 and kappa>=1 then the denominator is necessarily positive)



\subsection{Effects of circularity}
In this paragraph, we consider the Circular BP algorithm from \citet{Jardri2013} (i.e., Circular BP in the particular case $(\bm{\kappa}, \bm{\gamma}, \bm{\beta}) = (\bm{1}, \bm{1}, \bm{1})$) and look at the effects of circularity on the means and the precisions $\mu_i$ and $P_i$ of the belief or marginal distribution. The term ``circularity" is defined by $1-\alpha$, i.e., the distance to the value of $1$ which corresponds to BP (and is optimal for acyclic graphs, in which BP carries out exact inference).

First, increased amounts of circularity (that is, decreased $\alpha_{ij}$) % below the value $1$ corresponding to BP)
leads to increased precisions (or equivalently, smaller variance). This indicates an increased confidence in the beliefs. %compared to BP.
A mathematical justification is that $P_{i \to j}$ is an increasing function of all precisions of the incoming messages and of the circularity level ($1-\alpha$) as $g_{ij}$ is positive and increases as function of its argument $\sum_{k \in \mathcal{N}(i) \setminus j} P_{k \to i} + (1-\alpha_{ij}) P_{j \to i}$.
The increase in overconfidence %in precision  %of the beliefs
due to circularity in the Gaussian case %, associated to marginal probabilities and messages,
reminds the binary case, which had the same exact conclusions. % (see for instance Figure \ref{fig:CBP-overconfidence-acyclic}). 
This overconfidence effect is even increased in graphs with cycles, in which information not only reverberates within an edge ($i \to j \to i \to \dots$ because of $\alpha_{ij} \neq 1$, but also naturally through the cycles. Because all precisions are positive, it increases the already existing overconfidence brought by the circularity $1 - \alpha$. For a demonstration that BP overestimates precisions (or equivalently underestimates variances) in graphs with loops, see \citet{Weiss1999}.

As in the binary case, the effect of circularity seen in Gaussian Circular BP is not restricted to overconfidence but also to wrongness of the estimation (and potentially, of the subsequent decision). In the binary case, estimated beliefs (between 0 and 1) are not on the same side of the neutral value of 0.5, as shown in Figure \ref{fig:BP-and-CBP}. % and \ref{fig:CBP-overconfidence-acyclic}. 
In the Gaussian case, the estimation of the means $\{\mu_i\}$ depends on the value of $\alpha$ and is only approximate. Interestingly, \citet{Weiss1999} shows that means obtained by BP ($\bm{\alpha} = \bm{1}$) are exact if BP converges, even in graphs with cycles. Because function $h_{ij}$ determining $\abs{v_{i \to j}} \equiv P_{i \to j} \abs{\mu_{i \to j}}$ increases as function of its first argument and decreases as function of its second argument, and because $\mu$ can be negative, it is impossible to predict the evolution of $v_i = P_i \times \mu_i$ (nor the means $\mu_i$ themselves) with circularity. Nevertheless, simulations show that increased circularity (that is, decreased levels of $\alpha$) generally leads to more extreme estimations (i.e., increased absolute means $\abs{\mu_i}$) in addition to overestimated precisions, as shown in Figure \ref{fig:gaussian-CBP-overconfidence}.
%In the Gaussian case, not only there is increased confidence, but the estimation itself is impaired as the estimate means

\begin{figure}[h]
  \centering
%   \includesvg[width = 13.5cm]{Figures/Figure_networks_2_options}
%   \includegraphics[width = 13cm]{Figures/gaussian_network.pdf} %\linewidth
  \includegraphics[width = \linewidth]{Figures/GaussianCBP_means and precisions.pdf} %\linewidth
%  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace*{-3mm}
  \caption{\textbf{Effects of Circular BP %circularity 
  on the estimation of means and variances}. We consider an acyclic probabilistic graph and generate its weights (interactions between variables) and its inputs (unitary potentials) randomly. Full lines represent the best fitting polynomial function of degree 3. The black full line corresponds to identity.
%   \textbf{(A)} Function $g_{ij}$ on the precisions. 
%   \textbf{(B)} Function $h_{ij}$ on the potentials (precision $\times$ mean). 
%   \textbf{(C)} Estimated means increase in absolute value due to circularity. 
%   \textbf{(D)} Overconfidence brought by circularity, seen in the overestimation of the precisions.
  \textbf{(A)} Estimated means increase in absolute value due to circularity (that is, when $\alpha$ decreases from its value of 1 which corresponds to BP). Note that when applied on acyclic graphs as here, BP is exact; on acyclic graphs, BP only estimates exactly the means, not the precisions.
  \textbf{(B)} Circularity increases confidence, as Circular BP overestimates precisions for $\alpha < 1$ and underestimates them for $\alpha > 1$.
  }
  \label{fig:gaussian-CBP-overconfidence}
\end{figure}
% \afterPhD{TODO: generate figure \ref{fig:gaussian-CBP-overconfidence} and add it}

% \afterPhD{Discuss about overconfidence (precision) versus belief (estimation = mean).
% ``Biased" probabilistic inferences (actually depends: confidence vs estimation; see conclusions on binary vs gaussian).
% Note here that the confidence in ones' beliefs does not directly relate to the accuracy of the belief: one might have the correct belief given all the evidence at hand (and therefore take the right choice, e.g. getting vaccinated or not), but be more/less confident than what the evidence truly suggests. However, having disproportionate confidence on a systematic basis suggests that the reasoning machine itself it flawed and may sometimes lead to wrong beliefs. %these lines appear in the introduction chapter
% -----------> I should also talk about it in the binary case. Right beliefs = MAP problem (binary: I decide option A if option A looks better than option B / gaussian: I consider the highest probable option, e.g. speed of a car as measured by a radar). Have something about this in the conclusion chapter, including both the binary and the gaussian case+++. In general, for Circular BP, systematic overconfidence indicates a flawed reasoning overall, and therefore, the frequent presence of wrong beliefs and decisions.
% --> overconfidence tightly relates to wrong beliefs (i.e., taking wrong decisions)
% }


\subsection{Learning Gaussian CBP}
We present in this section the results of supervised learning of parameters of Circular BP on Gaussian probabilistic graphical models; see Figures \ref{fig:precisions-CBP-models-Erdos-Renyi} and \ref{fig:means-CBP-models-Erdos-Renyi}:

\paragraph{Simulated data}
Data for the training, validation and test sets were generated similarly to the binary case. For each connection probability $p$ ranging from $0.2$ to $1$, 30 weighted Erdos-Renyi graphs were generated with $n=9$ nodes. The weighting of each graph is controlled by variable $P_{x_i,x_j}$ ($2\times2$ precision matrix of factor $\psi_{ij}$), chosen randomly as follows: %\footnote{Explain why it was generated as such: what do $s_{ij}$ and $c_{ij}$ represent?}
\begin{equation}s_{ij} \sim \mathcal{U}([5; 10])\end{equation}
\begin{equation}J_{ij} \sim \mathcal{N}(\mu=0.5; \sigma=1)\end{equation}
\begin{equation}c_{ij} = \tanh(J_{ij}) s_{ij}\end{equation}
\begin{equation}Cov_{ij} = \begin{pmatrix} s_{ij} & c_{ij}\\ c_{ij} & s_{ij}\end{pmatrix}\end{equation}
\begin{equation}P_{x_i,x_j} = \frac{1}{s_{ij}^2 - c_{ij}^2} \begin{pmatrix}s_{ij} & -c_{ij}\\ -c_{ij} & s_{ij}\end{pmatrix}\end{equation}
The sign of the anti-diagonal coefficients of $P_{x_i,x_j}$ represents the sign of the interaction between $x_i$ and $x_j$ (similarly to Ising models, where it corresponds to the sign of variable $J_{ij}$).

Random inputs, controlled by variables $P_{\text{ext}, i}$, and $\mu_{\text{ext}, i}$ (precision and mean of factor $\psi_i$), were chosen randomly according to:
\begin{equation}P_{\text{ext}, i} \sim \text{Exp}(\lambda=3)\end{equation} %Exponential %exponential distribution %\mathcal{E}
\begin{equation}\mu_{\text{ext}, i} \sim \mathcal{N}(\mu=0; \sigma=1)\end{equation}
Exact marginals probability distributions (controlled by their precision $P$ and mean $\mu$) can be computed using linear algebra operations including matrix inversion \citep{Weiss1999}.

\paragraph{Supervised learning procedure}
For each weighted graph, 400 external inputs are generated (200 training examples, 100 validation examples, and 100 test examples). We minimize the KL-divergence between the true marginal distributions and the approximate ones:
\begin{align}
    \text{Cost} & = \sum_{\text{examples}} \sum_{i=1}^n D_{KL}(p_{\text{true,i}}\:, p_{\text{approx,i}}))\\
    & = \sum_{\text{examples}} \sum_{i=1}^n \Big[\log\Big(\frac{\sigma_\text{approx,i}}{\sigma_{\text{true,i}}}\Big) +  \frac{\sigma_{\text{true,i}}^2 + (\mu_{\text{true,i}} - \mu_\text{approx,i})^2}{2 \sigma_\text{approx,i}^2} - \frac{1}{2}\Big]  
\end{align}
where $i$ represent a node in the graph (among the $n=30$ nodes), or equivalently a variable $x_i$.
The fitting was carried out by the optimization procedure \emph{least squares} of SciPy \citep{SciPy2020}. %Scipy's optimization algorithm
All parameters $(\bm{\alpha}, \bm{\kappa}, \bm{\beta}, \bm{\gamma})$ are initialized at value $\bm{1}$.

% \paragraph{Unsupervised learning procedure}%not included because does not work (see longer comment below)
% We propose an unsupervised learning rule on parameter $\bm{\alpha}$ and $\bm{\kappa}$ (for $\bm{\beta}$ and $\bm{\gamma}$ at value $1$) in analogy to the one used for binary distributions (see section \ref{sec:unsupervised-learning-eCBP}). Parameter $\bm{\alpha}$ aims at decorrelating ``messages" and parameter $\bm{\kappa}$ aims at preventing reverberation of external information.\footnote{We do not consider the update equation of precisions $P_{i \to j}^{\text{new}} = g_{ij}(P_i - \alpha_{ij} P_{j \to i})$ and $P_i = \kappa_i (\sum_{j \in \mathcal{N}(i)} P_{j \to i} + P_{\text{ext} \to i})$ as precisions are positive numbers and therefore the same reasoning as for binary variables $M_{i \to j}$ (which can take positive or negative values) does not hold.}
% We use the equations $v_{i \to j}^{\text{new}} =  h_{ij}(v_i - \alpha_{ij} v_{j \to i},\, P_i - \alpha_{ij} P_{j \to i}) \propto v_i - \alpha_{ij} v_{j \to i}$ and $v_i = \kappa_i (\sum_{j \in \mathcal{N}(i)} v_{j \to i} + v_{\text{ext} \to i})$ to propose the following learning rules on $\bm{\alpha}$ and $\bm{\kappa}$:
% \begin{empheq}[left=\empheqlbrace]{align}%\label{}
%   &\Delta \alpha_{i \to j} = \eta_1 v_{j \to i}(v_i - \alpha_{i \to j} v_{j \to i})
%   \\
%   &\Delta \kappa_i = - \eta_2 v_{\text{ext} \to i} (v_i - v_{\text{ext} \to i})
% \end{empheq}
% with constant learning rates $\eta_1 = \eta_2 = 1e-5$ and 5000 training examples. Variables $v$ considered are taken after $T = 100$ iterations of Circular BP.
%----> Not included, as the unsupervised learning rule only marginally improves the performance of BP (in fact the learning rule on alpha decreases the performance so only the learning rule on kappa is used). The modified learning rule on kappa proposed by Sophie (see exchange of emails on 03/03/2022 for the intuition), $\Delta \kappa_i = - \eta_2 (v_{\text{ext} \to i} - (1-\kappa_i) v_i) (v_i - v_{\text{ext} \to i})$ (with parameter $\gamma_i$ used in Circular BP, but with $\gamma_i = 1/\kappa_i$) does not work either.

\paragraph{Results}

\begin{figure}[h]
  \centering
%   \includegraphics[width=\linewidth]{Figures/marginals_Erdos_Renyi_various.pdf} %marginals_Erdos_Renyi_eCBP.pdf
%   \includegraphics[width=\linewidth]{Figures/compressed_jpg/marginals_Erdos_Renyi_various} %marginals_Erdos_Renyi_eCBP
  \includegraphics[width=\linewidth]{Figures/ICML_precisions_Erdos_Renyi_eCBP_BP.pdf} %marginals_Erdos_Renyi_eCBP
%  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace*{-5mm}
  \caption{
  \textbf{Estimated precisions on the test set for BP and Circular BP}. %\textbf{Estimated marginals on the test set, for various trained algorithms}. 
  Probability distributions are represented by randomly generated Erdos-Renyi graphs with connection probabilities ranging from $0.2$ to $1$. For each connection probability, 30 randomly weighted graphs are considered (one example is shown on the first line of the figure), each with 200 external input examples in the training set and 100 in the test set. 
  Each point represents one node. For clarity, only one random node per graph is shown.
%   For BP, there is a sharp transition from carrying out rather good approximate inference for $p=0.2$ to performing really poorly for $p=0.3$ (at least on some of the 30 weighted graphs) because the system becomes frustrated.
  }
  \label{fig:precisions-CBP-models-Erdos-Renyi}
\end{figure}

\begin{figure}[h]
  \centering
%   \includegraphics[width=\linewidth]{Figures/marginals_Erdos_Renyi_various.pdf} %marginals_Erdos_Renyi_eCBP.pdf
%   \includegraphics[width=\linewidth]{Figures/compressed_jpg/marginals_Erdos_Renyi_various} %marginals_Erdos_Renyi_eCBP
  \includegraphics[width=\linewidth]{Figures/ICML_means_Erdos_Renyi_eCBP_BP.pdf} %marginals_Erdos_Renyi_eCBP
%  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace*{-5mm}
  \caption{
  \textbf{Estimated means on the test set for BP and Circular BP}. %\textbf{Estimated marginals on the test set, for various trained algorithms}. 
  Probability distributions are represented by randomly generated Erdos-Renyi graphs with connection probabilities ranging from $0.2$ to $1$. For each connection probability, 30 randomly weighted graphs are considered (one example is shown on the first line of the figure), each with 200 external input examples in the training set and 100 in the test set. 
  Each point represents one node. For clarity, only one random node per graph is shown.
%   For BP, there is a sharp transition from carrying out rather good approximate inference for $p=0.2$ to performing really poorly for $p=0.3$ (at least on some of the 30 weighted graphs) because the system becomes frustrated.
  }
  \label{fig:means-CBP-models-Erdos-Renyi}
\end{figure}

% \footnote{Add the unsupervised learning plots}

The Belief Propagation algorithm computes exact marginal means when the algorithm converges \citep{Weiss1999}, which was the case in all our simulations.%\footnote{how could have BP not converged?} 
Circular BP should therefore improve the quality of the approximate marginal precisions, while not worsening too much the quality of the means.
The supervised learning procedure indeed manages to improve substantially the approximate precisions (Figure \ref{fig:precisions-CBP-models-Erdos-Renyi}), while keeping the approximate means close to the exact ones (Figure \ref{fig:means-CBP-models-Erdos-Renyi}). 
% \footnote{Comment on the results of unsupervised learning in the Gaussian case}

==> Generalized_CBP.tex <==
%This file is not included in the final document. Indeed, I didn't manage to formulate a Generalized Circular BP (see explanation at the bottom of this .tex file).

%Generalized BP: Kikuchi approx = general case for Circular BP? If yes, then say it
%GBP vs Kikuchi: check that I didn't use "Kikuchi" when it was wrong. Try to define CBP using the Kikuchi approximation rather than the Bethe approximation
%Bethe case = two-layer region graph (see Example 1 in Loh2014) = any factor graph --> what is Kikuchi, does it correspond to clusters which are different from the original factors?



% \section{Generalized Circular BP}\label{sec:generalized-CBP}

% In this section, we present a generalized version of the Circular Belief Propagation algorithm, similarly to the Generalized Belief Propagation \citep{Yedidia2001, Yedidia2003, Yedidia2005}.

% Note that similarly to this section, one can define algorithms like Generalized BP and Circular BP on region graphs, a slightly more general form than factor graphs which considers sub- and super-regions; see \citet{Yedidia2001}. %Loh2014 %with potentially more layers than simply variable nodes (vertices) and hyperedges (factor nodes).


% \subsection{Generalized BP}
% \citet{Yedidia2005} provides a general method to yield extensions of BP. As for Circular BP, it is based the parametrization of BP's Bethe free energy to better approximate the Gibbs free energy.
% For higher performance, one can use the Kikuchi approximation rather than the Bethe approximation, which uses larger clusters of nodes, e.g. $b_{123}(x_1, x_2, x_3)$), to approximate the variational distribution $b(\mathbf{x})$. %and take clusters of variables (potentially more than two).
% \footnote{Talk more about Generalized BP: two things = introducing counting numbers + considering more regions than just the factor nodes and the variable nodes. Counting numbers = same approximation of the Gibbs free energy as used in this paper (Yedidia and colleagues inspect in more detail the case where counting numbers are 1, but let open using different counting numbers. + cite reweighted GBP?}

% \subsection{Generalized Circular BP}

% % In the main text, we use the same regions as in the Bethe approximation (see the Appendices for the general case)
% %entropic counting numbers $(\bm{\alpha}, \bm{\kappa})$ / average energy counting numbers $(\bm{\beta}, \bm{\gamma})$.


% \footnote{TODO: Work more on the link with Generalized BP from Yedidia}
% \footnote{Say that GBP has not been investigated using simulations: just a proposition from Yedidia.}

% This is a special case of \citet{Yedidia2005} which presents a method to build generalized BP algorithms based on such an approximation. We consider in this section the situation where the regions on which to make the approximation of the Gibbs free energy are simply the set of graph edges and individual nodes, as in the Bethe approximation (on the contrary, the key idea in Generalized BP is not only to reweight existing factors, but also to use larger groups of nodes within the Kikuchi approximation, e.g. $b_{123}(x_1, x_2, x_3)$). %; however, we consider the Kikuchi approximation in section \ref{sec:CBP-in-general-factor-graphs} which deals with the non-pairwise case). --> actually, we still consider the same factors as the ones from the probability distributions, be it in the pairwise case (this chapter) or the general case (last chapter)...

% where the Kikuchi approximation is a generalization of the Bethe approximation to larger groups of variables than pairs and singletons; see \citet{Yedidia2001}).

% Similarly to the pairwise factors case, Generalized Circular BP is defined as an approximation of Generalized reweighted BP \citep{Loh2014}, an extension of Generalized BP which uses a reweighted Kikuchi approximation.

% Note that the algorithm presented here is identical to the Generalized Belief Propagation algorithm of \citet{Yedidia2005}, with the minor difference that the work of Yedidia and colleagues focuses on so-called ``\emph{valid} region-based approximations" which imposes constraints between the counting numbers; these constraints are not considered in the present work. %\footnote{Precise the domain of $\beta_c$ and $\gamma_i$? I think $\in \mathbb{R}^*$ (but maybe $> 0$ only?)}

% \subsection{Tentative of derivation of Generalized Circular BP (failed)}
% Altogether, we obtain the following approximation of the Gibbs free energy $G_b^{\text{approx}} \approx G_b = U_b - S_b$:
% \begin{equation}\label{eq:modif-Bethe-Free-Energy-general}
%     G_b^{\text{approx}} = \sum\limits_{r \in R} \frac{1}{\alpha_r} \sum\limits_{\mathbf{x}_r} b_r(\mathbf{x}_r) \log\Bigg(\cfrac{b_r(\mathbf{x}_r)}{\prod\limits_{t \in \mathcal{C}(r)} b_t(\mathbf{x}_t)}\Bigg) - \sum\limits_{r \in R} \beta_r \sum\limits_{\mathbf{x}_r} b_r(\mathbf{x}_r) \log\Big(\psi_r(\mathbf{x}_r)\Big)
% \end{equation}
% We form the Lagrangian by adding Lagrange multipliers to $G_b^{\text{approx}}$. We obtain:
% \begin{equation}
%     \mathcal{L} = G_b^{\text{approx}} + \sum_{r \in R} \sum\limits_{t \in C(r)} \sum\limits_{x_t} \lambda_{rt}(\mathbf{x}_t) \Big(\sum\limits_{\mathbf{x}_r \setminus x_t} b_r(\mathbf{x}_r) - b_t(\mathbf{x}_t)\Big)
% \end{equation}
% The partial derivative of the Lagrangian is:
% \begin{equation}
%   \frac{\partial \mathcal{L}}{\partial b_r(\mathbf{x}_r)} = \frac{1}{\alpha_r} + \frac{1}{\alpha_c} \log\Bigg(\frac{b_c(\mathbf{x}_c)}{\prod\limits_{i \in \mathcal{N}(c)} b_i(x_i)}\Bigg) - \beta_c
% \log(\psi_c(\mathbf{x}_c)) + \sum\limits_{i \in \mathcal{N}(c)} \lambda_{c}(x_i) + \mu_c
% \end{equation}
% It comes, by cancelling the partial derivative of the Lagrangian:
% % ----------> If I write the Gibbs approximation using b_c(x_c)/prod_{i \ in \mathcal{N}(c)} b_i(x_i), then it is not possible to write explicitly the expression of $b_c(x_c)$ because it appears as log(b_c(x_c)) in one place, and 1/b_c(x_c) in another place (because of the denominator). So the only way to derive GBP (it seems) is to have only entropies, not mutual information as I do (= using a denominator). But then the resulting form of reweighted GBP is not as before (e.g. see Eq 16 of Loh2014), and we cannot propose a CBP algorithm out of it as in the pairwise case or the general factor graph case ----> Potential solution: see other derivations than Loh2014 of (reweighted) GBP, which could potentially make appear a formula for eFBP very similar to the factor graph case: this would allow for a definition of generalized CBP.
%I managed to have a formulation of Reweighted Generalized BP similar to BP and variants (see my manuscript papers "Generalized Circular BP" to take the derivations corresponding to Generalized BP (original work from Yedidia + reweighted Generalized BP by Loh2014) but there are multiple ways of modifying the message update equation to propose a Circular BP-like equation (see my manuscript papers + the comment of Eq 16 in Loh2014). So I decided not to define a Generalized Circular BP.

==> guess_sign_alpha_minus_1.tex <==
%For now this .tex file is not included in the Appendices
%TODO: remove occurences of "chapter"


Interestingly, cycles create what seems to be systematic overconfidence in BP (respectively systematic underconfidence, depending on the node considered); see Figure \ref{fig:BP-overconfidence-cyclic-graphs}. The sign of the bias (overconfidence or underconfidence) can partly be guessed. As a matter of fact, the quantity that determines whether information is amplified or attenuated in a cycle is the product of edge weights over the cycle $\prod_{\text{cycle}} J_{\text{edge}}$. The propagation of messages is indeed determined by function $f(x, J) = \arctanh(\tanh(J) \tanh(x))$ which has the same sign as $J \times x$. Therefore, a message entering node $i$ travels in the cycle before coming back to the same node $i$, with a weight whose sign is $\sgn(\prod_{\text{cycle}} J_{\text{edge}})$. Therefore, the belief at node $i$ is overconfident if $\prod_{\text{cycle}} J_{\text{edge}} > 0$, and underconfident otherwise. In fact, function $f$ can be linearized with $f(x, J) \approx J \times x$. As a consequence, $\prod_{\text{cycle}} J_{\text{edge}}$ not only gives the sign of the amplification, but it also represents the level of amplification of the message by the cycle. Note that this way of predicting the sign of the bias (overconfidence or underconfidence) only works for graphs with a single cycle. With multiple cycles possibly including identical edges, a first approximation would be to sum each contribution of all cycles passing through node $i$ with $\sum_{\text{cycles}} \prod_{\text{cycle}} J_{\text{edge}}$ and consider its sign, but this is sometimes not right because of the non-linearities in the system. %overcounting (because of double counting as the information travels through the cycle and comes back)
%the sign of the product of weights $J$ determines whether there is amplification i.e. overcounting, or undercounting: $f(x, J)$ has the same sign as $J xl$.


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/overconfidence_BP_cyclic_graphs.pdf}
%   \includesvg[width=\linewidth]{Figures/overconfidence_BP_cyclic_graphs}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace*{-3mm}
  \caption{\textbf{Systematic bias (overconfidence or underconfidence, depending on the node) is observed when applying the Belief Propagation algorithm to a cyclic graph}. The direction of the bias is determined by the local structure around the node. For instance, the blue node belongs to a \emph{positive cycle} (that is, a cycle for which the product of the weights $J_{ij} > 0$) and therefore produces overconfident beliefs due to double counting, and the green node belongs to a \emph{negative cycle} and therefore produces underconfident beliefs.}
  \label{fig:BP-overconfidence-cyclic-graphs}
\end{figure}



% As studied in section \ref{sec:CBP-as-model-of-impaired-behavior}
As shown previously in Figure \ref{fig:CBP-overconfidence-acyclic} for acyclic graphs, Circular Belief Propagation also creates overconfidence in all nodes of the graph. More specifically, the choice of the circularity level in Circular BP leads to whether overconfidence (for $\alpha < 1$ in acyclic graphs, which was the initial idea behind explaining circular inferences) or underconfidence (for $\alpha > 1$ in acyclic graphs).
What comes from these observations is the idea that in cyclic graphs, the right level of circularity in Circular BP could improve the inference compared to standard BP, by counteracting the effect of cycles.

\paragraph{Improving the quality of inference with Circular BP}
For instance, if all graph weights are positive, BP is overconfident on all nodes, and ``anti-Circular BP" (i.e., Circular BP with $\alpha > 1$) causes some underconfidence, (partly) compensating for the overconfidence created by cycles; see Figure \ref{fig:CBP-cycle-positive-weights-fighting-overconfidence}. Figure \ref{fig:CBP-uniform-alpha-different-graph-types}B shows that the estimation of the marginal probability by Circular BP is best around $\alpha = 1.2$ (a second example is also shown in the same plot for a different random graph). In graphs with only positive weights, the optimal uniform $\alpha$ is always $>1$, because all cycles contribute to overcounting the same information several times.

\begin{figure}%[H]
  \centering
%   \includegraphics[width=\linewidth]{Figures/anti_Circular_BP_vs_exact_marginals.pdf}
  \includegraphics[width=\linewidth]{Figures/compressed_jpg/anti_Circular_BP_vs_exact_marginals}
%   \includesvg[width=\linewidth]{Erdos_Renyi}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace*{-4mm}
  \caption{\textbf{How Circular BP could fight the effect of loops}. In this example, weights of the (cyclic) graph $J_{ij}$ are taken all positive, and Circular BP is applied to the graph with $\bm{\alpha}$ taken uniformly over the edges. Because of the positive weights, the marginals approximated by BP (case $\alpha = 1$) are overconfident. However, underconfidence brought by (anti-)Circular BP partly compensates for the overconfidence naturally originating from the graph cycles. There is an ``optimal" value for $\alpha$ (here $\alpha_{\text{opt}} \approx 1.2$, for which beliefs are not overconfident ($\alpha < \alpha_{\text{opt}}$) nor underconfident ($\alpha > \alpha_{\text{opt}}$). The graph was randomly generated and randomly weighted. 300 examples $\bm{M_{\text{ext}}}$ were randomly generated. One point represents the approximate marginal under Circular BP versus exact marginal, for each node and each example. The full line represents the average of all points. See Figure \ref{fig:CBP-overconfidence-acyclic} for acyclic graphs instead.}%from applying BP to a cyclic graph.
  \label{fig:CBP-cycle-positive-weights-fighting-overconfidence}
\end{figure}

In graphs with only negative weights, cycles with length 3 (which are the smallest possible cycles and have more impact in general compared to cycles of higher length) contribute to undercounting information as the product of the weights $J_{ij}$ over such cycles is negative. For this reason, the optimal $\alpha$ is (nearly) always $<1$ for such graphs, as shown in Figure \ref{fig:CBP-uniform-alpha-different-graph-types}C.

Finally, and most interestingly, for graphs with both positive and negative weights chosen randomly, the optimal level of circularity $\alpha$ in the graph is often close to $1$ (where $\bm{\alpha}$ is as before taken uniformly); see Figure \ref{fig:CBP-uniform-alpha-different-graph-types}D. This comes from having both \emph{negative cycles} and \emph{positive cycles}, where the sign of a cycle is by definition the sign of the product of the weights $J_{ij}$ over this cycle. Positive and negative cycles have different effects. Negative cycles may lead to oscillations while running the BP algorithm. Positive cycles may amplify noisy or random initial messages and therefore have incorrect convergence values of the beliefs, which depend on the sign of the initial conditions, and on the graph structure rather than on the external input value itself.

\begin{figure}%[H]
  \centering
  \includegraphics[width=\linewidth]{Figures/CBP_MSE_vs_alpha_different_graphs.pdf}
%   \includesvg[width=\linewidth]{Erdos_Renyi}
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \vspace*{-4mm}
  \caption{\textbf{How to choose $\bm{\alpha}$ in Circular BP to fight the effect of loops}. The log-error between the exact probability and the belief obtained from Circular BP are computed depending on parameter $\bm{\alpha}$ used in Circular BP (here $\bm{\alpha}$ is taken uniformly over the edges, equal to $\alpha$). Two random graphs are considered, except for panel A (one random graph).
  \textbf{(A)} In random trees, BP is an exact algorithm, thus the optimal value for $\alpha$ is $1$.
  \textbf{(B)} In random graphs with positive weights, BP is overconfident as all cycles are positive, thus the optimal value for $\alpha$ is $>1$. The curve peaking around $\alpha = 1.2$ represents the graph of Figure \ref{fig:CBP-cycle-positive-weights-fighting-overconfidence}.
  \textbf{(C)} In random graphs with negative weights and high enough density, BP is underconfident as the smallest cycles (length 3) are always negative, thus the optimal value for $\alpha$ is $<1$.
  \textbf{(D)} In random graphs with both positive and negative weights, the existence of both positive and negative cycles makes the optimal $\alpha$ be $<1$ or $>1$, depending on the random graph.
  }
  \label{fig:CBP-uniform-alpha-different-graph-types}
\end{figure}

Non-uniform $\bm{\alpha}$ can even improve the quality of inference more than for uniform $\bm{\alpha}$. The optimal amount of \emph{local} circularity $\alpha_{ij}$ in Circular BP (associated to edge $(x_i, x_j)$ in the probabilistic graph) depends on the local structure around the edge. If the edge ($x_i$, $x_j$) belongs to a positive cycle then marginals estimated by BP for nodes $x_i$ and $x_j$ are overconfident and $\alpha_{ij}$ should be $>1$ to compensate for it. Conversely, if the edge belongs to a negative cycle then marginals estimated by BP for $x_i$ and $x_j$ are underconfident and $\alpha_{ij}$ should be $<1$. Of course, in practice edges belong to several cycles of different signs and strengths (product of weights) thus it can be complicated to predict on which side of $1$ parameter $\alpha_{ij}$ should be.

\paragraph{Goal of this chapter}%\footnote{This is rather a summary of the chapter... --> should go into the summary??}
In this chapter, we use Circular BP in order to counterbalance the amount of ``natural" overcounting %to reduce the amount of overcounting 
In cyclic graphs, ``anti-Circular BP" prevents the systematic overcounting observed with BP.
More specifically, we show that appropriate amounts of \emph{local} circularity $\alpha_{ij}$ in Circular BP (where $\alpha_{ij}$ is associated to edge $(x_i, x_j)$ in the probabilistic graph) can improve the quality of inference. In this state, information is transmitted accurately, without ``explosion" of the system (overamplification) nor ``shutting down" of the system (overdampening). 


\paragraph{Organization of this chapter}
This chapter is organized as follows. In section \ref{sec:CBP-as-approximate-FBP}, we provide a theoretical justification to Circular BP (which was initially defined through intuition rather than from normative principles): %whose definition did not come from normative principles but instead intuition: 
Circular BP is an approximation to Fractional BP, which was proposed in \citet{Wiegerinck2002} as an approximate inference method extending BP. In section \ref{sec:extension-of-CBP}, we propose a generalization of the Circular BP from \citet{Jardri2013} (also called the Circular BP algorithm) based on an extension of Fractional BP (Reweighted BP). After showing that it is possible to guarantee the convergence of the new algorithm in section \ref{sec:conv-results}, we show through simulations in section \ref{sec:learning-CBP} that it is possible to learn the parameters of Circular BP in a supervised manner, so that it performs approximate inference accurately.
Finally, in section \ref{sec:CBP-with-memory}, we propose an algorithm, ``Circular BP with memory", similar to Circular BP, but which more closely relates to the initial idea of cancelling messages being reverberated through the cycles of the graph.
